Team ACK at SemEval-2025 Task 2: Beyond Word-for-Word Machine Translation for English-Korean Pairs

Translating knowledge-intensive and entity-rich text between English and Korean requires transcreation to preserve language-specific and cultural nuances beyond literal, phonetic or word-for-word conversion. We evaluate 13 models (LLMs and MT models) using automatic metrics and human assessment by bilingual annotators. Our findings show LLMs outperform traditional MT systems but struggle with entity translation requiring cultural adaptation. By constructing an error taxonomy, we identify incorrect responses and entity name errors as key issues, with performance varying by entity type and popularity level. This work exposes gaps in automatic evaluation metrics and hope to enable future work in completing culturally-nuanced machine translation.

==> tables/average_entity_score.tex <==
\definecolor{bleuColor}{HTML}{E0B7B7}
\definecolor{cometColor}{HTML}{94BFA7}
\definecolor{metaColor}{HTML}{E2C391}


\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccc}
        \hline
        & \multicolumn{3}{c}{\textbf{Metrics}} \\
        \textbf{Models} & \it{BLEU} & \it{COMET} & \it{M-ETA} \\
        \hline
        \it{o1} & \cellcolor{bleuColor} 0.3869 & 0.9196 & 0.3752 \\
        \it{o1 Mini} & 0.3830 & \cellcolor{cometColor} 0.9202 & 0.3306 \\
        \it{GPT-4o} & 0.3692 & 0.9087 & 0.3951 \\
        \it{GPT-4o Mini} & 0.3545 & 0.9046 & 0.2914 \\
        \it{Claude 3.5 Sonnet} & 0.1961 & 0.8384 & 0.3969 \\
        \it{Claude 3.5 Haiku} & 0.1584 & 0.8056 & 0.2849 \\
        \it{Gemini 1.5 Pro} & 0.3810 & 0.9094 & \cellcolor{metaColor} 0.4833 \\
        \it{Gemini 1.5 Flash} & 0.2965 & 0.9081 & 0.3316 \\
        \it{Grok 2} & 0.3808 & 0.9143 & 0.3514 \\
        \it{DeepSeek R1} & 0.0066 & 0.4895 & 0.0026 \\
        \it{Llama 3} & 0.0327 & 0.5529 & 0.0563 \\
        \it{Mbart-50} & 0.1451 & 0.8702 & 0.0791 \\
        \it{NLLB-200} & 0.2195 & 0.8899 & 0.1663 \\
        \hline
    \end{tabular}
    }
    \caption{Automatic evaluation results on BLEU, COMET, and M-ETA for English-Korean translation.}
    \textbf{Color key:} 
    \textcolor{black}{\fboxsep0.5pt\colorbox{bleuColor}{\rule{0pt}{6pt}\rule{6pt}{0pt}}} = Highest BLEU,
    \textcolor{black}{\fboxsep0.5pt\colorbox{cometColor}{\rule{0pt}{6pt}\rule{6pt}{0pt}}} = Highest COMET,
    \textcolor{black}{\fboxsep0.5pt\colorbox{metaColor}{\rule{0pt}{6pt}\rule{6pt}{0pt}}} = Highest M-ETA.
    \label{tab:results}
\end{table}


%Maybe, could you align this to the right side? Make this a single column table. just needs to be tightened up. Info is good.
